When Is a Relation Worth Trusting? Manipulation Costs, Exposure, and the Trust Trap in Multi-Relational Graph Learning

Multi-relational graph detectors learn from clean data how much to trust each relation, but an adversary pays a different price to manipulate each relation and each action; taking such costs as given, we ask when using a relation is worse than ignoring it. Our first main result proves that degree gating strictly beats every selection or reweighting of a relation when part of the population is isolated on it and the attacker cannot afford to open the gate, and that this window is sharp; on real graphs, validated gating gains exactly on the relations that meet these conditions and nowhere else. Our second shows that a per-node exposure bound, which extends to message passing, tells a platform which relation to harden: exposure per unit cost, computed without any attack, picks the relation whose hardening raises the exact trap threshold most in 15 of 16 cases, against at most 7 for informativeness, cheapness, or an analysis with equal edit costs. Supporting tools give exact worst cases for linear relational models, certified brackets for R-GCN and tree ensembles, and a finite-sample guarantee for adversarial validation, under which clean-trained graph detectors fall below their graph-free counterparts in 58 of 90 settings on six graphs. A selection protocol built on these results is never significantly worse than ignoring the graph; with at most four relations it mostly abstains, as validation alone would, and its cost-aware proposals help when relations are many, so far shown on synthetic graphs. Without cost information, the safe choice is to abstain.

==> tables/tab_doubt.tex <==
Standard (3 seeds) & \underline{.043} & \textbf{.836} & .836 & \underline{.442} & \textbf{.935} & .935\\
No label oracle & \underline{.055} & \textbf{.835} & .836 & \underline{.434} & \textbf{.933} & .935\\
Black box (surrogate) & \underline{.237} & \textbf{.835} & .836 & \underline{.742} & \textbf{.933} & .935\\
Entity-level, Q1 (3 seeds) & \underline{.520} & \textbf{.837} & .837 & \underline{.777} & \textbf{.935} & .935\\
Sybil accounts, $c_s{=}1$ & \underline{.040} & \textbf{.835} & .835 & \underline{.058} & \textbf{.933} & .933\\
Persistent camouflage & \underline{.601} & \textbf{.835} & .835 & \underline{.866} & \textbf{.933} & .933\\
Features ($\epsilon{=}0.05$) + structure & \underline{.050} & \textbf{.767} & .767 & \underline{.315} & \textbf{.749} & .749\\
10\% training labels & \underline{.097} & \textbf{.800} & .800 & \underline{.427} & \textbf{.893} & .893\\
S-FFSD, temporal split (3 seeds) & \underline{.145} & \textbf{.560} & .560 & \underline{.186} & \textbf{.593} & .593\\

